TuniQ: Autotuning Compilation Passes for Quantum Workloads at Scale for Effectiveness and Efficiency

Quantum processors are being integrated into HPC ecosystems as co-processors, where compilation of quantum circuits into hardware-executable form determines both output fidelity and runtime. Current compilers use a fixed pass sequence and ignore the fact that optimal pass selection varies with circuit, hardware, and noise conditions. We present TuniQ, a reinforcement learning-based system that selects compilation passes at each pipeline stage, adapting to circuit, backend, and current noise profile. TuniQ introduces several novel design components like a dual-encoder for stage-aware representation, shaped rewards for cross-stage credit assignment, and dynamic action masking for valid compilation. Evaluated across diverse quantum workloads on multiple IBM Quantum Cloud processors, TuniQ improves fidelity and reduces compilation time over the state-of-the-art IBM Qiskit transpiler, generalizes across backends without retraining, and scales strongly to utility-scale circuits with growing advantage.

==> design_old.tex <==
\section{Design}

\subsection{Problem Formulation}

We formulate quantum circuit compilation as a  Decision Process $\mathcal{M} = (S, A, T, R, \gamma)$
where the agent sequentially selects transpiler passes to transform an input circuit.

\subsubsection{State Space}

The state $s_t \in \mathcal{S}$ at timestep $t$ comprises:
\begin{itemize}
    \item The current circuit $C_t$ (represented via extracted features)
    \item The current compilation stage $k \in \{0, 1, \ldots, 5\}$
    \item Pass application history within the current episode
    \item Backend noise characteristics
\end{itemize}

\subsubsection{Action Space}

At each timestep, the agent selects an action $a_t$ from the set of valid passes for the current stage, plus a ``skip'' action to advance to the next stage:

\begin{equation}
    \mathcal{A}_k = \mathcal{P}_k \cup \{\texttt{skip}\}
\end{equation}

where $\mathcal{P}_k$ is the set of candidate passes for stage $k$. For optimization stages (4 and 5), we use subset selection where the agent chooses a subset of passes to apply together:

\begin{equation}
    \mathcal{A}_{k \in \{4,5\}} = 2^{|\mathcal{P}_k|} \cup \{\texttt{skip}\}
\end{equation}

\subsubsection{Transition }

applying pass $p$ to circuit $C_t$ yields $C_{t+1} = p(C_t)$. The ``skip'' action advances the stage counter without modifying the circuit.

\subsubsection{Action Masking}

Not all actions are valid at every state. We employ action masking to enforce:
\begin{itemize}
    \item \textbf{Stage constraints}: Only passes appropriate for the current stage are available.
    \item \textbf{Dependency constraints}: Some passes require prerequisites (e.g., routing requires layout).
    \item \textbf{Minimum/maximum pass limits}: Each stage has bounds on pass applications.
    \item \textbf{Failure tracking}: Routing passes that fail on a circuit are masked for subsequent attempts.
\end{itemize}

The mask $M_t \in \{0,1\}^{|\mathcal{A}|}$ is computed dynamically based on the current state.

\subsection{Compilation Pipeline}

Our compilation pipeline consists of six stages, allowing learned flexibility within each stage.

\subsubsection{Stage 0: Initialization (Fixed)}

For now the in the initialization stage we are  applying a fixed sequence of passes to prepare the circuit to reduce the infinite action space at this stage. We will extend this stage in our RL pipeline to all the available passes. Currently the following passes are applied and then we start our RL pipeline from Layout stage
\begin{enumerate}
    \item \texttt{Unroll3qOrMore}: Decompose 3+ qubit gates.
    \item \texttt{UnrollCustomDefinition}: Decompose Custom Definitions.
    \item \texttt{RemoveIdentityEquivalent}: Remove identity gates.
    \item \texttt{CommutativeCancellation}: Cancel commuting gate pairs.
    \item \texttt{ConsolidateBlocks}: Merge consecutive unitaries.
    \item \texttt{UnitarySynthesis}: Resynthesize unitary blocks.
\end{enumerate}

This stage is not learned, ensuring circuits enter the RL-controlled stages in a canonical form. 

\subsubsection{Stage 1: Layout Selection}

The agent selects a layout algorithm to map logical qubits to physical qubits:

 
\begin{equation}
    \begin{split}
        \mathcal{P}_1 = \{ & \texttt{VF2Layout}, \texttt{SabreLayout}, \texttt{DenseLayout}, \\
        & \texttt{TrivialLayout}, \texttt{CSPLayout}\}
    \end{split}
\end{equation}



\subsubsection{Stage 2: Routing}

After layout, the agent selects routing algorithms to insert SWAP gates for connectivity:

\begin{equation}
    \mathcal{P}_2 = \{\texttt{SabreSwap}, \texttt{LookaheadSwap}, \texttt{BasicSwap}, \texttt{VF2PostLayout}\}
\end{equation}

This stage uses a two-substage structure:
\begin{enumerate}
    \item \textbf{Substage 0}: Select a routing algorithm (not \texttt{VF2PostLayout})
    \item \textbf{Substage 1}: Optionally apply \texttt{VF2PostLayout} to improve the mapping
\end{enumerate}

\subsubsection{Stage 3: Basis Translation (Fixed)}

Basis translation converts all gates to the backend's native gate set. This stage is mandatory and not learned:

\begin{equation}
    \mathcal{P}_3 = \{\texttt{BasisTranslation}\}
\end{equation}

The translation pipeline includes \texttt{UnitarySynthesis},  \newline
 \texttt{HighLevelSynthesis}, \texttt{BasisTranslator}, and \texttt{GateDirection} to ensure all gates are in basis and correctly oriented.

\subsubsection{Stage 4: Optimization}

The agent selects subsets of optimization passes to apply iteratively until convergence:

\begin{equation}
\mathcal{P}_4 = \left\{
    \begin{array}{l}
        \texttt{ConsolidateBlocks}, \texttt{UnitarySynthesis}, \\
        \texttt{RemoveIdentityEquivalent},  \\
        \texttt{Optimize1qGatesDecomposition}, \\
        \texttt{CommutativeCancellation}, \\
        \texttt{ContractIdleWiresInControlFlow}
    \end{array} 
\right\}
\end{equation}

Out of the given passes, the agents selects a subset of passes and keep applying untill there is no improvement in gates and depth. 


\subsubsection{Stage 5: Final Cleanup}

A final optimization stage for last-pass cleanup:


\begin{equation}
    \mathcal{P}_5 = \left\{
      \begin{array}{l}
        \texttt{Optimize1qGatesDecomposition} \\
        \texttt{CommutativeCancellation} \\
        \texttt{RemoveIdentityEquivalent} \\
        \texttt{VF2PostLayout}
       \end{array}
    \right\}
\end{equation}

\subsection{Observation Space}

We design a hybrid observation space that provides different representations depending on the compilation stage, reflecting the fundamentally different nature of pre-layout (logical) and post-routing (physical) structures of  circuits.

\subsubsection{Stage Indicator}

A one-hot vector $\mathbf{s} \in \{0,1\}^6$ indicating the current stage.

\subsubsection{Circuit Features}

\paragraph{Pre-Layout Features (Stages 0-2)}

Before routing, the circuit operates on logical qubits without physical placement. We encode the circuit as a 4D tensor:

For two-qubit gates:
\begin{equation}
    \mathbf{F}^{2Q} \in \mathbb{R}^{Q \times Q \times G \times T \times 1}
\end{equation}

where $Q$ is the maximum logical qubits (20), $G$ is the number of gate types (20), and $T$ is the number of temporal bins (5). Each entry counts gates of type $g$ between qubits $i,j$ in time bin $t$.

For single-qubit gates:
\begin{equation}
    \mathbf{F}^{1Q} \in \mathbb{R}^{Q \times G \times T \times 1}
\end{equation}

The temporal binning is computed by assigning each gate to a bin based on its depth in the DAG:
\begin{equation}
    \text{bin}(g) = \left\lfloor \frac{\text{depth}(g)}{\text{total\_depth}} \cdot T \right\rfloor
\end{equation}

\paragraph{Post-Routing Features (Stages 3-5)}

After routing, the circuit is mapped to physical qubits with noise characteristics. We encode with additional channels:

For two-qubit gates:
\begin{equation}
    \mathbf{F}^{2Q} \in \mathbb{R}^{E \times G \times T \times 4}
\end{equation}

where $E$ is the number of coupling edges (352 for IBM backends). The four channels are:
\begin{enumerate}
    \item Gate count
    \item Two-qubit gate error rate $\epsilon_{2Q}(e)$ for edge $e$
    \item Average $T_1$ coherence of the two qubits
    \item Average $T_2$ coherence of the two qubits
\end{enumerate}

For single-qubit gates:
\begin{equation}
    \mathbf{F}^{1Q} \in \mathbb{R}^{P \times G \times T \times 5}
\end{equation}

where $P$ is the number of physical qubits (156). The five channels encode gate count, two single-qubit gate error rates, $T_1$, and $T_2$.

\subsubsection{Global Features}
A vector $\mathbf{g} \in \mathbb{R}^{80}$ containing circuit metrics, topology analysis, and compatibility indicators. The features are organized into four groups:

\paragraph{Circuit Metrics (14 dimensions)}
\begin{itemize}
    \item \textbf{Gate counts} (normalized): total gates $/1000$, single-qubit gates $/1000$, two-qubit gates $/1000$
    \item \textbf{Structural metrics}: depth $/100$, width $/127$
    \item \textbf{Derived ratios}: depth-to-gate ratio $\frac{\text{depth}}{\text{total\_gates}}$, two-qubit gate fraction $\frac{N_{2Q}}{N_{\text{total}}}$
    \item \textbf{Parallelism}: average gates per layer, maximum parallelism $/10$
    \item \textbf{Quality}: Estimated Success Probability (ESP) when available after basis translation
    \item \textbf{Stage flags}: binary indicators for pre-layout stage, post-routing stage, and basis-translated state
    \item \textbf{Basis compatibility}: fraction of gates already expressed in the target basis gate set
\end{itemize}

\paragraph{Circuit Topology (6 dimensions)}
We construct an interaction graph $G_C = (V_C, E_C)$ where vertices represent logical qubits and edges connect qubits that interact via two-qubit gates. We extract:
\begin{equation}
    \mathbf{t}_C = \left[ \frac{d(G_C)}{30}, \frac{\Delta(G_C)}{10}, \frac{\bar{\delta}(G_C)}{5}, \rho(G_C), \frac{k(G_C)}{10}, \frac{|C_{\max}|}{|V_C|} \right]
\end{equation}
where $d$ is diameter, $\Delta$ is maximum degree, $\bar{\delta}$ is average degree, $\rho$ is edge density, $k$ is the number of connected components, and $|C_{\max}|$ is the size of the largest connected component.

\paragraph{Backend Topology (6 dimensions)}
The same six metrics computed for the backend coupling graph $G_B$:
\begin{equation}
    \mathbf{t}_B = \left[ \frac{d(G_B)}{30}, \frac{\Delta(G_B)}{10}, \frac{\bar{\delta}(G_B)}{5}, \rho(G_B), \frac{k(G_B)}{10}, \frac{|C_{\max}|}{|V_B|} \right]
\end{equation}
These values are cached after first computation since the backend topology remains constant.

\paragraph{Compatibility Ratios (4 dimensions)}
Circuit-to-backend ratios that indicate mapping difficulty:
\begin{equation}
    \mathbf{r} = \left[ \frac{d(G_C)}{d(G_B)}, \frac{\Delta(G_C)}{\Delta(G_B)}, \frac{\rho(G_C)}{\rho(G_B)}, \frac{\bar{\delta}(G_C)}{\bar{\delta}(G_B)} \right]
\end{equation}
Values greater than 1.0 indicate the circuit topology is more demanding than the backend can naturally accommodate, suggesting potential routing overhead.

The remaining dimensions are zero-padded for  fixed size of 80.

\newpage


\subsubsection{Pass History Features}

\paragraph{Recent Pass Sequence (5 dimensions)}
The last 5 applied passes encoded as normalized vocabulary indices:
\begin{equation}
    h_i = \frac{\text{idx}(p_{-(i})}{\left| V \right|}, \quad i \in \{1, 2, 3, 4,5\}
\end{equation}
where ${V}$ is the pass vocabulary constructed from all candidate passes across stages, and $p_{-k}$ denotes the $k$-th most recent pass. 
for example we applied $[pass X , ....., Pass A, Pass B, none, none, none]$ 
and idx(Pass A) = 40 , idx (Pass B) = 50 and total passes = 100 then
our $embedding\_vector  = [0.4, 0.5, 0, 0, 0]$

\paragraph{No-op Counts (7 dimensions)}
Consecutive no-operation counts for key optimization passes, normalized by a maximum of 5: 
So here the 7 dimensions are hardcoded for the following 7 passes listed below since these are the ones that 
are frequently used in the convergence check. 

\begin{equation}
    h_{5+j} = \min\left(\frac{n_{\text{noop}}(p_j)}{5}, 1.0\right)
\end{equation}
for passes $p_j$ in the array
$P = [\texttt{ConsolidateBlocks},\\
\phantom{P = [}\texttt{UnitarySynthesis},\\
\phantom{P = [}\texttt{Optimize1qGates},\\
\phantom{P = [}\texttt{Optimize1qGatesDecomposition},\\
\phantom{P = [}\texttt{CommutativeCancellation},\\
\phantom{P = [}\texttt{InverseCancellation},\\
\phantom{P = [}\texttt{RemoveIdentityEquivalent}]$
A pass is marked as a no-op when it produces no change to the circuit. High no-op counts signal diminishing returns, guiding the agent to skip or advance stages.

\paragraph{Stage Progress (1 dimension)}
The number of passes applied in the current stage, normalized:
\begin{equation}
    h_{13} = \frac{n_{\text{stage}}}{30}
\end{equation}

The remaining dimensions are zero-padded to 128.



\subsubsection{Context Features}
For providing optimization progress indicators and detailed mapping quality assessment.

\paragraph{Optimization State (13 dimensions)}
\begin{itemize}
    \item  fraction of gates in target basis
    \item  normalized depth $/100$, depth-to-gate ratio
    \item  normalized 1Q count $/100$, normalized 2Q count $/100$, 2Q fraction, 1Q fraction
    \item  gate reduction ratio $\frac{N_{\text{initial}} - N_{\text{current}}}{N_{\text{initial}}}$, depth reduction ratio $\frac{D_{\text{initial}} - D_{\text{current}}}{D_{\text{initial}}}$
    \item  pre-layout flag, post-routing flag, basis-translated flag, layout-exists flag
\end{itemize}

\paragraph{Mapping Quality (8 dimensions, post-layout only)}
After routing, to analyze the quality of the current qubit mapping:
\begin{itemize}
    \item  For each two-qubit gate, we compute the coupling graph distance between its operands. We report mean path length $/10$, maximum path length $/20$, and the fraction of gates with path lengths of exactly 1, exactly 2, and $\geq 3$.
    \item  Maximum gate count on any single physical qubit, normalized by 50.
    \item \textbf{Error concentration}: Fraction of two-qubit gates placed on edges in the worst 20\% and worst 10\% by error rate:
    \begin{equation}
        f_{80} = \frac{|\{g : \epsilon(e_g) \geq \epsilon_{80}\}|}{N_{2Q}}, \quad f_{90} = \frac{|\{g : \epsilon(e_g) \geq \epsilon_{90}\}|}{N_{2Q}}
    \end{equation}
    where $\epsilon_{80}$ and $\epsilon_{90}$ are the 80th and 90th percentile error thresholds across all coupling edges.
\end{itemize}

\paragraph{Improvement Potential (6 dimensions, post-layout only)}
Metrics indicating whether remapping (e.g., via \texttt{VF2PostLayout}) could improve circuit quality:
\begin{itemize}
    \item \textbf{Unused good edges}: Fraction of low-error edges (below median) not currently utilized
    \item \textbf{Error ratio}: $\frac{\bar{\epsilon}_{\text{used}}}{\bar{\epsilon}_{\text{unused}}}$, comparing average error of used vs. unused edges
    \item \textbf{Qubit utilization}: Fraction of physical qubits used, and its complement (available capacity)
    \item \textbf{Spatial spread}: $\frac{\max(Q_{\text{used}}) - \min(Q_{\text{used}})}{N_{\text{physical}}}$, measuring how dispersed the mapping is across the device
    \item \textbf{Edge utilization}: Fraction of coupling edges with at least one gate
\end{itemize}

For pre-layout stages (before routing), the mapping quality and improvement potential dimensions are set to zero.

\subsection{Neural Network Architecture}


\subsubsection{Dual Circuit Encoder}

The circuit features pass through one of two encoders based on stage:

\paragraph{Pre-Layout Encoder (Stages 0-2)}
\begin{equation}
    \phi_{\text{pre}}(\mathbf{F}) = \text{MLP}_{2048 \rightarrow 1024 \rightarrow 512 \rightarrow 256}(\text{flatten}(\mathbf{F}))
\end{equation}

\paragraph{Post-Routing Encoder (Stages 3-5)}
\begin{equation}
    \phi_{\text{post}}(\mathbf{F}) = \text{MLP}_{2048 \rightarrow 1024 \rightarrow 512 \rightarrow 256}(\text{flatten}(\mathbf{F}))
\end{equation}

Both use ReLU activations and 10\% dropout.

\subsubsection{Auxiliary Encoders}

% \begin{itemize}
%     \item \textbf{Pass History Encoder}: $\text{MLP}_{256 \rightarrow 128}$ producing 128-dim embedding
%     \item \textbf{Context Encoder}: $\text{MLP}_{128 \rightarrow 64}$ producing 64-dim embedding
%     \item \textbf{Global Encoder}: $\text{MLP}_{128 \rightarrow 64}$ producing 64-dim embedding
%     \item \textbf{Stage Embedding}: Learned 32-dim embedding per stage
% \end{itemize}

\subsubsection{Combined Representation}

% The final observation embedding concatenates all components:
% \begin{equation}
%     \mathbf{z} = [\phi_{\text{circuit}}(\mathbf{F}); \phi_{\text{history}}(\mathbf{h}); \phi_{\text{context}}(\mathbf{c}); \phi_{\text{global}}(\mathbf{g}); \mathbf{e}_{\text{stage}}] \in \mathbb{R}^{544}
% \end{equation}

\subsubsection{Policy and Value Networks}

% The embedding feeds into separate policy and value heads:
% \begin{align}
%     \pi(a|s) &= \text{softmax}(\text{MLP}_{256 \rightarrow 256}(\mathbf{z})) \odot M_t \\
%     V(s) &= \text{MLP}_{256 \rightarrow 256 \rightarrow 1}(\mathbf{z})
% \end{align}

% where $M_t$ is the action mask and $\odot$ denotes masking invalid actions.

\subsection{Reward Design}

Our reward function provides dense feedback by comparing against a deterministic teacher baseline computed for each circuit.

\subsubsection{Transpilation Guide}

For each training circuit, we compute a helper baseline by executing a fixed sequence set of passes that almost ties with Qiskit L3 Preset Pass manager in terms of ESP. 

Why compare with a Helper baseline during each stage and at the end with ESP of \qbest?

We cannot blindly trust the ESP. ESP of a 2-Qubit Circuit with a far worse optimization choice can be much higher than ESP of a 10-Qubit Circuit with a very optimal pass selection. As the Qubit Number and Number of gates grow, ESP reduces. But could we normalize based on these values?
Actually No. Since ESP is not a function of just Circuit structure, it depends on which region the circuit is mapped to, the current noise profile of the backend where the circuit is being mapped, and the graph structure and edge error of the backend, since the number of SWAPS also varies as the Backend changes. 
So Blindly ESP is not trustworthy unless it is consistently compared against a very fixed baseline with the same backend and the same noise profile . 
Using a comparison against a fixed baseline cancels out factors outside the agent's control. 
So the system reflects only the marginal output of the pass selection, rather than the current noise profile or ever-changing backends and circuit structures across different episodes during training. 


The fixed pass sequences are as follows.
\begin{enumerate}
    \item The fixed init passes that we used in the RL
    \item \textbf{Layout}: Try VF2Layout, fall back to SabreLayout
    \item \textbf{Routing}: Apply SabreSwap if needed, then VF2PostLayout
    \item \textbf{Optimization}: Run the Qiskit Level 3 convergence loop
    \item \textbf{Clean up}: Fixed 3 clean up passes. 
\end{enumerate}

This provides stage-wise targets: $\{\text{ESP}_k^{\text{teacher}}, \text{gates}_k^{\text{teacher}}, \text{depth}_k^{\text{teacher}}\}$ for each stage $k$.

\subsubsection{Stage-Wise Rewards}

Each stage computes rewards by comparing RL metrics against teacher baseline using a bounded log-ratio:

\begin{equation}
    r_{\text{ESP}} = \alpha \cdot \frac{\log(\text{ESP}_{\rl} / \text{ESP}_{\text{teacher}})}{\sqrt{1 + \log^2(\text{ESP}_{\rl} / \text{ESP}_{\text{teacher}})}}
\end{equation}



\paragraph{Stage 1 (Layout)}
We compute a proxy ESP that estimates post-routing fidelity based on predicted SWAP costs:
\begin{equation}
    r_1 = \alpha_{\text{ESP}} \cdot f(\text{ESP}_{\text{proxy}}^{\rl}, \text{ESP}_{\text{proxy}}^{\text{teacher}}) + \alpha_{\text{swap}} \cdot \frac{\text{swaps}^{\text{teacher}} - \text{swaps}^{\rl}}{\text{swaps}^{\text{teacher}}}
\end{equation}

\paragraph{Stage 2 (Routing)}
\begin{equation}
    r_2 = \alpha_{\text{ESP}} \cdot f(\text{ESP}_{\text{proxy}}^{\rl}, \text{ESP}_{\text{proxy}}^{\text{teacher}}) + \alpha_g \cdot \frac{g^{\text{teacher}} - g^{\rl}}{g^{\text{teacher}}} + \alpha_d \cdot \frac{d^{\text{teacher}} - d^{\rl}}{d^{\text{teacher}}}
\end{equation}

\paragraph{Stages 4-5 (Optimization)}
After basis translation, we compute actual ESP:
\begin{equation}
    r_{4,5} = \alpha_{\text{ESP}} \cdot f(\text{ESP}^{\rl}, \text{ESP}^{\text{teacher}}) + \alpha_g \cdot \frac{g^{\text{teacher}} - g^{\rl}}{g^{\text{teacher}}} + \alpha_d \cdot \frac{d^{\text{teacher}} - d^{\rl}}{d^{\text{teacher}}}
\end{equation}

\subsubsection{Final Reward}

At episode termination, we compute a final reward comparing against Qiskit Level 3:
\begin{equation}
    r_{\text{final}} = w_{\text{ESP}} \cdot f(\text{ESP}^{\rl}, \text{ESP}^{L3}) + w_{2Q} \cdot \Delta_{2Q} + w_d \cdot \Delta_d + w_{1Q} \cdot \Delta_{1Q} + r_{\text{quality}}
\end{equation}

where $\Delta$ terms are normalized differences and $r_{\text{quality}}$ penalizes circuits with non-basis gates or custom definitions.

\subsubsection{No-Op Penalties}

To discourage repeated ineffective pass applications, we penalize no-ops (passes that don't change the circuit):
\begin{equation}
    r_{\text{noop}} = -\beta_{\text{base}} \cdot n_{\text{noop}}^{\beta_{\text{exp}}} \cdot \gamma_{\text{consec}}^{\max(0, n_{\text{consec}} - 2)}
\end{equation}

where $n_{\text{noop}}$ is the count of no-ops for this pass and $n_{\text{consec}}$ is consecutive no-ops.

\subsection{Training Procedure}

\subsubsection{Algorithm}

We use Maskable Proximal Policy Optimization (PPO) from Stable-Baselines3 with the following hyperparameters:

\begin{table}[h]
\centering
\caption{PPO Hyperparameters}
\begin{tabular}{ll}
\toprule
Parameter & Value \\
\midrule
Learning rate & $3 \times 10^{-4}$ \\
Batch size & 128 \\
Number of epochs & 10 \\
Number of steps & 2048 \\
Discount factor $\gamma$ & 0.99 \\
GAE $\lambda$ & 0.95 \\
Clip range & 0.2 \\
Entropy coefficient & 0.01 \\
Value function coefficient & 0.5 \\
Max gradient norm & 0.5 \\
\bottomrule
\end{tabular}
\end{table}

\subsubsection{Multi-Backend Training}

To improve generalization, we train on multiple perturbed backend variants. Starting from a base backend (e.g., IBM Pittsburgh), we generate $N$ perturbations by:
\begin{enumerate}
    \item Jittering $T_1/T_2$ coherence times by $\pm 20\%$
    \item Jittering gate error rates by $\pm 15\%$
\end{enumerate}

During training, environments rotate through backends in a strided round-robin pattern, ensuring each environment sees different backends across episodes.

\subsubsection{Circuit Generation}

Training circuits are generated randomly with:
\begin{itemize}
    \item Qubit count: uniformly sampled from $[5, 15]$
    \item Depth: $2n$ to $5n$ where $n$ is qubit count
    \item Gates: random 1Q and 2Q gates with measurements
\end{itemize}

Each circuit is preprocessed with 
$Unroll3qOrMore$ and \newline
$UnrollCustomDefinitions$ before entering the RL environment.\\

\subsubsection{Parallel Environments}

We use 8 parallel SubprocVec environments, with rolling checkpoints (keeping last 5) to manage disk space during long training runs.

\begin{algorithm}[t]
\caption{Multi-Stage RL Circuit Compilation}
\begin{algorithmic}[1]
\STATE \textbf{Input:} Circuit $C$, Backend $B$, Policy $\pi_\theta$
\STATE \textbf{Output:} Compiled circuit $C'$
\STATE
\STATE $C \leftarrow \textsc{Preprocess}(C)$ \COMMENT{Unroll, remove identities}
\STATE $s \leftarrow \textsc{InitState}(C, B)$
\STATE $k \leftarrow 1$ \COMMENT{Start at layout stage}
\STATE
\WHILE{$k \leq 5$}
    \STATE $M \leftarrow \textsc{ComputeMask}(s, k)$
    \STATE $a \sim \pi_\theta(\cdot | s) \odot M$
    \IF{$a = \texttt{skip}$}
        \IF{$k = 4$} 
            \STATE $C \leftarrow \textsc{RetranslateBasis}(C)$ \COMMENT{If needed}
        \ENDIF
        \STATE $k \leftarrow k + 1$
    \ELSIF{$k \in \{4, 5\}$}
        \STATE $P \leftarrow \textsc{DecodeSubset}(a)$
        \REPEAT
            \FOR{$p \in P$}
                \STATE $C \leftarrow p(C)$
            \ENDFOR
        \UNTIL{no improvement}
    \ELSE
        \STATE $p \leftarrow \textsc{DecodePass}(a, k)$
        \STATE $C \leftarrow p(C)$
    \ENDIF
    \STATE $s \leftarrow \textsc{UpdateState}(s, C)$
\ENDWHILE
\STATE
\RETURN $C$
\end{algorithmic}
\end{algorithm}

\section{Experimental Setup}

\subsection{Backends}

We evaluate on IBM Quantum backends:
\begin{itemize}
    
    \item \textbf{IBM Brisbane}: 127 qubits, heavy-hex topology
\end{itemize}


\subsection{Baselines}

We compare against:
\begin{itemize}
    \item \textbf{Qiskit Level 0}: Minimal compilation 
    \item \textbf{Qiskit Level 1}: Light optimization
    \item \textbf{Qiskit Level 2}: Medium optimization with noise-aware layout
    \item \textbf{Qiskit Level 3}: Heavy optimization with multiple iteration loops
\end{itemize}

\subsection{Evaluation Metrics}

\begin{itemize}
    \item \textbf{ESP}: Expected Success Probability (primary metric)
    \item \textbf{Two-Qubit Gate Count}: Number of 2Q gates
    \item \textbf{Circuit Depth}:  
    \item \textbf{One-Qubit Gate Count}: 
    \item \textbf{Compilation Time}: Wall-clock time excluding model inference
    \item \textbf{Win Rate}: Percentage of circuits where RL beats baseline
\end{itemize}

\subsection{Evaluation Protocol}

For evaluation, we:
\begin{enumerate}
    \item Generate a held-out test set of 500 random circuits
    \item Compile each circuit with RL agent (greedy action selection) and all baselines
    \item Compute ESP and structural metrics for each compiled circuit
\end{enumerate}

To ensure fair comparison:
\begin{itemize}
    \item Qiskit baselines use seed 42 for determinism
    \item Compilation time measurements exclude RL inference time
    \item ESP is computed using the same backend target for all methods
\end{itemize}

\subsection{Training Configuration}

\begin{itemize}
    \item Total timesteps: 1,000,000
    \item Number of perturbed backends: 30
    \item Maximum episode steps: 200
    \item Action timeout: 10 seconds per pass
\end{itemize}

